Efficient variable-length hanging tether parameterization for marsupial robot planning in 3D environments

This paper presents a novel approach to efficiently parameterize and estimate the state of a hanging tether for path and trajectory planning of a UGV tied to a UAV in a marsupial configuration. Most implementations in the state of the art assume a taut tether or make use of the catenary curve to model the shape of the hanging tether. The catenary model is complex to compute and must be instantiated thousands of times during the planning process, becoming a time-consuming task, while the taut tether assumption simplifies the problem, but might overly restrict the movement of the platforms. In order to accelerate the planning process, this paper proposes defining an analytical model to efficiently compute the hanging tether state, and a method to get a tether state parameterization free of collisions. We exploit the existing similarity between the catenary and parabola curves to derive analytical expressions of the tether state.

==> 06-Results_Opt_table_old.tex <==
\begin{table*}[t!]
\caption{Results for catenary approach  taken from \cite{smartinezr2023}, related to computing time optimization, distance to obstacles, and trajectory time parameters in simulated environments. SI: Scenario; F: Feasibility [\%]; TCO: Time for optimized solution [$s$];  DPOO: Distance parable obstacles optimized[$m$]; DOO: Distance obstacles optimized[$m$]; VTO: Velocity, optimized trajectory [$m/s$]; ATO: Acceleration, optimized trajectory [$m/s^2$]} 
\centering
\label{tab:experiments_old}
\small
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|ll|ll|llllll|llllll|}
\hline
\multicolumn{3}{|c}{\textbf{ALL}} &
\multicolumn{2}{|c}{\textbf{CATENARY}} &
\multicolumn{6}{|c}{\textbf{UGV}} & 
\multicolumn{6}{|c|}{\textbf{UAV}} \\ 
\hline
\multicolumn{1}{|c}{\textbf{SI}} & 
\multicolumn{1}{|c}{\textbf{F}} & 
\multicolumn{1}{|c}{\textbf{TCO}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ DCOO\end{tabular}}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Min\\ DCOO\end{tabular}}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ DOO\end{tabular}}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Min\\ DOO\end{tabular}}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ VTO\end{tabular}}} & 
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Max\\ VTO\end{tabular}}} & 
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ ATO\end{tabular}}} & 
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Max\\ ATO\end{tabular}}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ DOO\end{tabular}}} &
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Min\\ DOO\end{tabular}}} & 
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ VTO\end{tabular}}} & 
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Max\\ VTO\end{tabular}}} & 
\multicolumn{1}{|c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ ATO\end{tabular}}} & 
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Max\\ ATO\end{tabular}} \\
\hline
S1.1 &  86.0 & 465.9 & 1.14 & 0.25 & 2.28 & 1.55 & 0.36 & 1.07 & 0.02 & 0.81  & 1.87 & 0.80 & 0.97 & 1.19 & -0.002 & -0.09 \\
S1.2 &  80.0 & 529.7 & 1.31 & 0.16 & 3.76 & 1.60 & 0.43 & 1.25 & 0.02 & 0.78  & 2.21 & 0.89 & 0.91 & 1.19 & -0.002 & -0.08 \\
S2.1 &  94.5 & 123.6 & 0.72 & 0.10 & 0.69 & 0.56 & 0.13 & 0.91 & 0.02 & 0.96  & 1.19 & 0.76 & 1.01 & 1.15 & 0.002  & 0.01  \\
S2.2 &  95.0 & 109.3 & 0.75 & 0.13 & 0.75 & 0.58 & 0.19 & 1.00 & 0.03 & 1.09  & 1.16 & 0.67 & 0.99 & 1.09 & 0.000  & 0.07  \\
S3.1 &  84.8 & 213.6 & 0.67 & 0.13 & 0.98 & 0.62 & 0.50 & 1.07 & 0.00 & 0.21  & 0.81 & 0.56 & 1.02 & 1.21 & 0.003  & 0.16  \\
S3.2 &  84.0 &214.9 & 0.67 & 0.14 & 0.97 & 0.61 & 0.55 & 1.08 & 0.00 & -0.20 & 0.79 & 0.54 & 0.98 & 1.16 & 0.004  & 0.18  \\
S4.1 &  82.5 & 539.0 & 0.74 & 0.14 & 2.12 & 1.40 & 0.45 & 1.14 & 0.02 & 1.00  & 1.16 & 0.65 & 0.94 & 1.12 & -0.002 & -0.06 \\
S4.2 &  76.0 & 708.6 & 0.76 & 0.10 & 1.70 & 1.07 & 0.47 & 1.32 & 0.01 & 0.86  & 1.15 & 0.65 & 0.92 & 1.22 & -0.002 & -0.32 \\
S5.1 &  98.0 & 277.8 & 1.09 & 0.23 & 2.26 & 0.76 & 0.41 & 1.15 & 0.03 & 1.07  & 1.74 & 0.83 & 0.97 & 1.27 & -0.004 & -0.14 \\
S5.2 &  95.0 & 447.7 & 1.14 & 0.22 & 2.53 & 0.63 & 0.57 & 1.08 & 0.02 & 1.02  & 1.66 & 0.65 & 0.92 & 1.11 & -0.004 & -0.12\\
\hline
\end{tabular}
\end{adjustbox}
\vspace*{-2mm}
\end{table*}

==> algorithm.tex <==

\begin{algorithm}
  \caption{Recursive algorithm for finding a collision-free parable}
  \label{alg:parable}
  \begin{algorithmic}
  
    \Require $A,B \in \Re^2$
    \Require Parable:    $ y = ax^2 + bx + c$
    \Require $[a,b,c] \in \Re^3$
    \Require $C_{obs}=\cup_{i_1}^NO_i$ obstacles in the environment
    \Require $N$ Number of obstacles in the environment
    
    \If{$a=b=c=0$}
      \State $a\gets0$ // First iteration 
      \State Calculate b and c such as the parable is the line that passes through $A$ and $B$
    \EndIf

    \State{$C_{intersect} = \emptyset$}
    \For{$O \in C_{obs}$}
    \If{$Parable$ intersects with $O$}
    \State{$C_{intersect}=C_{intersect} \cup O$}
    \EndIf
    \EndFor

    \If{$C_{intersect}=\emptyset$}
    \Return{Parable}
    
    \Return{parable(A,B,[a,b,c])}
  
    \EndIf
  
  \end{algorithmic}
\end{algorithm}

@INPROCEEDINGS{8468627,
  author={Xiao, Xuesu and Fan, Yiming and Dufek, Jan and Murphy, Robin},
  booktitle={2018 IEEE International Symposium on Safety, Security, and Rescue Robotics (SSRR)}, 
  title={Indoor UAV Localization Using a Tether}, 
  year={2018},
  volume={},
  number={},
  pages={1-6},
  keywords={Unmanned aerial vehicles;Robot sensing systems;Azimuth;Gravity;Cameras},
  doi={10.1109/SSRR.2018.8468627}}

